The Complex Multi-Wavelength Morphology of the Peculiar Compact Galaxy Group IC 2431

We present new Chandra X-ray imaging spectroscopy of the compact galaxy group IC 2431, and compare with archival ultraviolet, optical, infrared, and radio images. IC 2431 is a starburst system containing three tidally-distorted disk galaxies. All three galaxies may have active nuclei. One galaxy is classified as an AGN based on its optical spectrum, a second is identified as a possible X-ray AGN based on the Chandra data, and the third galaxy may host a radio AGN. In optical images, a prominent dust lane crosses the southern galaxy, while Spitzer infrared images show a dusty bridge connecting the two brightest galaxies. Chandra maps reveal a massive (2 x 10^7 M(sun)) concentration of hot gas between these two galaxies, as well as several other knots of hot gas and non-thermal emission. The unabsorbed X-ray luminosity of the hot gas in IC 2431 is ~ 1 x 10^42 erg/s, which is enhanced by about a factor of four relative to the star formation rate, compared to other star-forming galaxies. In radio maps, a bright jet/ridge of radio continuum emission extends 4 kpc from one nucleus. We compare the properties of IC 2431 with those of other interacting galaxy systems, and discuss two different scenarios that may account for the peculiarities of IC 2431: ram pressure stripping of the interstellar medium during a head-on collision between two galaxies, or an AGN-powered radio jet that has been distorted by an interaction with interstellar gas during a tidal encounter between galaxies.

==> xspec_gas_table1.tex <==
\begin{deluxetable}{cccccccccc}
\tablecolumns{10}
\tablewidth{0pc}
\caption{Chandra Spectral Results for the X-Ray Sources within IC 2431\label{xspectab_gas}}
\tablehead{   
\colhead{X-Ray}   
& \colhead{RA}
& \colhead{DEC}
& \colhead{radius}
& \colhead{NH}
& \colhead{kT}    
& \colhead{$\Gamma$} 
& \colhead{C-statistic/DOF}
&\colhead{APEC}
&\colhead{Power Law}\\ 
\colhead{Source} 
&\colhead{(deg)} 
&\colhead{(deg)} 
&\colhead{($''$)} 
&\colhead{$\times$10$^{22}$}
& \colhead{(keV)}    
&\colhead{} 
& \colhead{}
& \colhead{Log L$_{\rm X}$}
& \colhead{Log L$_{\rm X}$}
\\ 
\colhead{ID} 
&&&
& \colhead{(cm$^{-2}$)}
& \colhead{}    
& \colhead{}
& \colhead{}
& \colhead{(0.3-8 keV)}
& \colhead{(0.3-8 keV)}
\\ 
\colhead{} 
&&
& \colhead{}
& \colhead{}    
& \colhead{}
& \colhead{}
& \colhead{}
& \colhead{(erg~s$^{-1}$)}
& \colhead{(erg~s$^{-1}$)}
\\ 
\colhead{} 
&&
& \colhead{}
& \colhead{}    
& \colhead{}
& \colhead{}
& \colhead{}
& \colhead{(unabsorbed)}
& \colhead{(unabsorbed)}
\\ 
}
\startdata
{\bf \#1  }& 136.14752 & 14.59499 & 1.7
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 32.33/26 & 38.83 $\pm$ $_{0.16}^{0.07}$ & 40.44 $\pm$ $_{0.09}^{0.08}$\\
\#1 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 32.33/26 & 39.37 $\pm$ $_{0.13}^{0.06}$ & 40.44 $\pm$ $_{0.08}^{0.1}$\\
\#1 &  &  & 
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 32.11/26 & 39.9 $\pm$ $_{0.12}^{0.13}$ & 40.45 $\pm$ $_{0.16}^{0.09}$\\
{\bf \#2  }& 136.14657 & 14.59378 & 1.7
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 8.31/21 & 40.43 $\pm$ $_{0.07}^{0.08}$ & 39.95 $\pm$ $_{0.08}^{0.1}$\\
\#2 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 8.12/21 & 40.69 $\pm$ $_{0.07}^{0.08}$ & 40.04 $\pm$ $_{0.11}^{0.08}$\\
\#2 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 9.47/21 & 40.8 $\pm$ $_{0.11}^{0.07}$ & 40.14 $\pm$ $_{0.09}^{0.09}$\\
\#2 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 8.27/21 & 41.09 $\pm$ $_{0.1}^{0.09}$ & 40.08 $\pm$ $_{0.12}^{0.07}$\\
{\bf \#3  }& 136.14574 & 14.59329 & 1.5
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 41.7/51 & 40.29 $\pm$ $_{0.07}^{0.06}$ & 40.7 $\pm$ $_{0.07}^{0.06}$\\
\#3 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 43.04/51 & 39.53 $\pm$ $_{0.04}^{0.07}$ & 40.71 $\pm$ $_{0.06}^{0.06}$\\
\#3 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 42.39/51 & 40.42 $\pm$ $_{0.06}^{0.07}$ & 40.73 $\pm$ $_{0.07}^{0.05}$\\
\#3 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 41.6/51 & 40.91 $\pm$ $_{0.06}^{0.05}$ & 40.76 $\pm$ $_{0.09}^{0.06}$\\
{\bf \#4  }& 136.14509 & 14.59290 & 1.3
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 8.1/13 & 40.33 $\pm$ $_{0.09}^{0.1}$ & 39.64 $\pm$ $_{0.09}^{0.11}$\\
\#4 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 7.97/13 & 40.63 $\pm$ $_{0.12}^{0.08}$ & 39.72 $\pm$ $_{0.11}^{0.1}$\\
\#4 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 7.49/13 & 40.8 $\pm$ $_{0.11}^{0.11}$ & 39.82 $\pm$ $_{0.15}^{0.09}$\\
\#4 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 7.94/13 & 41.02 $\pm$ $_{0.13}^{0.11}$ & 39.8 $\pm$ $_{0.11}^{0.13}$\\
{\bf \#5  }& 136.14488 & 14.59385 & 2.0
& 0.04  frozen & 2  frozen & 1.6  frozen & 59.02/25 & 40.53 $\pm$ $_{0.03}^{0.14}$ & 35.8 $\pm$ $_{0.03}^{0.17}$\\
\#5 &  &  & 
& 0.04  frozen & 0.04 $\pm$ -0.99 & 1.6  frozen & 76.33/25 & 39.56 $\pm$ $_{0.02}^{2.43}$ & 39.3 $\pm$ $_{0.04}^{0.11}$\\
\#5 &  &  & 
& 0.04  frozen & 1.5  frozen & 1.6  frozen & 55.36/25 & 40.61 $\pm$ $_{0.05}^{0.11}$ & 70.51 $\pm$ $_{2.16}^{0.14}$\\
\#5 &  &  & 
& 0.04  frozen & 1.3  frozen & 2  frozen & 54.46/26 & 40.63 $\pm$ $_{0.04}^{0.13}$ & 38.48 $\pm$ $_{0.04}^{0.13}$\\
\#5 &  &  & 
& 0.04  frozen & 1.3  frozen & 1.6  frozen & 54.4/25 & 40.66 $\pm$ $_{0.05}^{0.13}$ & 36.8 $\pm$ $_{0.05}^{0.11}$\\
\#5 &  &  & 
& 0.04  frozen & 1.3  frozen & 2  frozen & 54.49/25 & 40.69 $\pm$ $_{0.03}^{0.12}$ & 36 $\pm$ $_{0.03}^{0.14}$\\
\#5 &  &  & 
& 0.04  frozen & 1  frozen & 2  frozen & 54.64/25 & 40.83 $\pm$ $_{0.1}^{0.1}$ & 39.71 $\pm$ $_{0.11}^{0.08}$\\
\#5 &  &  & 
& 0.04  frozen & 1  frozen & 1.6  frozen & 54.56/25 & 40.84 $\pm$ $_{0.07}^{0.1}$ & 39.63 $\pm$ $_{0.09}^{0.09}$\\
\#5 &  &  & 
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 55.45/25 & 40.96 $\pm$ $_{0.09}^{0.1}$ & 0 $\pm$ $_{0.04}^{0}$\\
\#5 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 56.28/25 & 41.06 $\pm$ $_{0.12}^{0.07}$ & 40.07 $\pm$ $_{0.11}^{0.12}$\\
\#5 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 57.6/25 & 41.23 $\pm$ $_{0.15}^{0.11}$ & 40.22 $\pm$ $_{0.16}^{0.07}$\\
{\bf \#6  }& 136.14466 & 14.59569 & 1.6
& 0 $\pm$ 0.87 & 0.43 $\pm$ 0.95 & 2.01 $\pm$ 0.62 & 43.47/58 & 40.52 $\pm$ $_{0.58}^{-0.09}$ & 40.6 $\pm$ $_{0.49}^{-0.06}$\\
\#6 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 44.58/60 & 40.97 $\pm$ $_{0.11}^{0.04}$ & 40.66 $\pm$ $_{0.1}^{0.04}$\\
\#6 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 43.62/60 & 41.22 $\pm$ $_{0.11}^{0.06}$ & 40.69 $\pm$ $_{0.1}^{0.06}$\\
{\bf \#7  }& 136.14412 & 14.59513 & 1.2
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 47.53/34 & 37.28 $\pm$ $_{0.12}^{0.05}$ & 40.46 $\pm$ $_{0.13}^{0.04}$\\
\#7 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 46.73/35 & 40.2 $\pm$ $_{0.09}^{0.09}$ & 40.55 $\pm$ $_{0.05}^{0.08}$\\
\#7 &  &  & 
& 0.04  frozen & 1  frozen & 1.6  frozen & 45.4/35 & 40.28 $\pm$ $_{0.1}^{0.07}$ & 40.47 $\pm$ $_{0.07}^{0.05}$\\
\#7 &  &  & 
& 4.5 $\pm$ 4.06 & 34.56 $\pm$ 306.64 & 9.5 $\pm$ 6.3 & 39.74/32 & 40.25 $\pm$ $_{0.76}^{0.16}$ & 40.01 $\pm$ $_{0}^{-0.18}$\\
\#7 &  &  & 
& 0.04  frozen & 1  frozen & 1.6  frozen & 43.4/34 & 40.84 $\pm$ $_{0.08}^{0.1}$ & 0 $\pm$ $_{0.04}^{0}$\\
\#7 &  &  & 
& 0.04  frozen & 1  frozen & 1.6  frozen & 43.4/34 & 40.83 $\pm$ $_{0.1}^{0.05}$ & 0 $\pm$ $_{0}^{0}$\\
\#7 &  &  & 
& 0.04  frozen & 1  frozen & 1.6  frozen & 43.4/34 & 40.83 $\pm$ $_{0.1}^{0.05}$ & 0 $\pm$ $_{0}^{0}$\\
\#7 &  &  & 
& 0.04  frozen & 0.8  frozen & 1.6  frozen & 43.82/34 & 40.97 $\pm$ $_{0.14}^{0.11}$ & 40.41 $\pm$ $_{0.1}^{0.07}$\\
{\bf \#8  }& 136.14361 & 14.59463 & 1.2
& 0.04  frozen & 1  frozen & 1.6  frozen & 18.15/21 & 40.35 $\pm$ $_{0.12}^{0.1}$ & 40.17 $\pm$ $_{0.15}^{0.07}$\\
\#8 &  &  & 
& 0.04  frozen & 0.6  frozen & 1.6  frozen & 17.02/22 & 40.56 $\pm$ $_{0.1}^{0.08}$ & 40.21 $\pm$ $_{0.09}^{0.08}$\\
\#8 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 17.47/22 & 40.72 $\pm$ $_{0.11}^{0.09}$ & 40.25 $\pm$ $_{0.12}^{0.08}$\\
\#8 &  &  & 
& 0.04  frozen & 0.4  frozen & 1.6  frozen & 16.43/22 & 41.01 $\pm$ $_{0.07}^{0.1}$ & 40.24 $\pm$ $_{0.09}^{0.08}$\\
\enddata
\end{deluxetable}

